Location Aggregation of Spatial Population CTMC Models

In this paper we focus on spatial Markov population models, describing the stochastic evolution of populations of agents, explicitly modelling their spatial distribution, representing space as a discrete, finite graph. More specifically, we present a heuristic approach to aggregating spatial locations, which is designed to preserve the dynamical behaviour of the model whilst reducing the computational cost of analysis. Our approach combines stochastic approximation ideas (moment closure, linear noise), with computational statistics (spectral clustering) to obtain an efficient aggregation, which is experimentally shown to be reasonably accurate on two case studies: an instance of epidemic spreading and a London bike sharing scenario.

==> eptcsdata.tex <==
\providecommand{\firstpage}{30}
\providecommand{\publicationstatus}{M. Tribastone and H. Wiklicky (Eds.): International Workshop on\\Quantitative Aspects of Programming Languages and Systems (QAPL'16)\\
EPTCS 227, 2016, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.227.3}{10.4204/EPTCS.227.3}}
\pdfoutput=1

